FISHDBC: Flexible, Incremental, Scalable, Hierarchical Density-Based Clustering for Arbitrary Data and Distance

FISHDBC is a flexible, incremental, scalable, and hierarchical density-based clustering algorithm. It is flexible because it empowers users to work on arbitrary data, skipping the feature extraction step that usually transforms raw data in numeric arrays letting users define an arbitrary distance function instead. It is incremental and scalable: it avoids the $\mathcal O(n^2)$ performance of other approaches in non-metric spaces and requires only lightweight computation to update the clustering when few items are added. It is hierarchical: it produces a "flat" clustering which can be expanded to a tree structure, so that users can group and/or divide clusters in sub- or super-clusters when data exploration requires so. It is density-based and approximates HDBSCAN*, an evolution of DBSCAN.

==> figures/tab-internal.tex <==
% tab:internal
\begin{table*}[htbp]
    \newcommand{\cfill}{\xrfill[2.5pt]{0.05pt}}
    \newcommand{\oom}{\multicolumn{7}{c}{\cfill\textit{Out of memory}\cfill}}
    \centering
    %\footnotesize
    \begin{adjustbox}{max width=\textwidth}
    % \rowcolors{8}{gray!15}{}
    \begin{tabular}{lrrrrrrrrr}
        \toprule
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Size} & \multirow{2}{*}{Algorithm (\ef)} & \multicolumn{2}{c}{Clustered elements} & \multicolumn{2}{c}{Clusters} & \multirow{2}{*}{Silhouette} & \multicolumn{2}{c}{Average distance} \\
        \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){9-10}
        & & & flat & hierarchical & flat & hierarchical & & intra-cluster & inter-cluster  \\
        \midrule
        % & 
        % %   &  10 &     390 &        946 &     5 &    12 &     0.055 &     0.384 &     0.675 \\
        %   & \FISHDBC (20) & \bf 398 & \bf 1\ 546 &     4 &    10 &     0.509 &     0.381 & \bf 0.882 \\
        %  & & \FISHDBC (50) &     385 &        995 &     3 &     6 &     0.513 &     0.381 &     0.871 \\
        % %  & & 100 &     385 &        999 &     3 &     6 &     0.512 &     0.381 &     0.870 \\
        % %  & & 200 &     372 &        372 & \bf 2 & \bf 4 &     0.518 &     0.382 &     0.857 \\
        % \multirow{-3}{*}{DW-Kos}  & \multirow{-3}{*}{3\ 430} &  \HDBSCAN &     353 &        353 & \bf 2 & \bf 4 & \bf 0.532 & \bf 0.375 &     0.854 \\
        % %  & &  NG &     524 &         -- &     5 &    -- &           &      0.63 &      0.80 \\
        % \midrule
        \multirow{3}{*}{DW-Enron} & \multirow{3}{*}{39\ 861}
        %   &  10 &      5\ 405 &     31\ 707 & \bf 194 & \bf 408 &     0.245 &     0.499 &     0.963 \\
           & \FISHDBC (20) &      6\ 094 &     36\ 039 & \bf 222 & \bf 454 & \bf 0.552 & \bf 0.301 &     0.969 \\
         & & \FISHDBC (50) &      6\ 340 &     34\ 408 &     238 &     486 &     0.549 &     0.309 &     0.969 \\
        %  & & 100 &      6\ 387 &     35\ 458 &     237 &     484 &     0.549 &     0.312 &     0.970 \\
        %  & & 200 &      6\ 361 &     35\ 866 &     239 &     488 &     0.545 &     0.314 &     0.970 \\
         & &  \HDBSCAN & \bf  7\ 206 & \bf 39\ 344 &     299 &     642 &     0.469 &     0.326 & \bf 0.973 \\
        %  & &  NG &     10\ 167 &          -- &    1206 &      -- &           &     0.18  &     0.65  \\
        \midrule
        \multirow{3}{*}{DW-NYTimes} & \multirow{3}{*}{300\ 000} 
        %   &  10 &     26\ 370 &     301\ 179 & \bf 752 & \bf 1\ 574 & &     0.593 &     0.965 \\
           & \FISHDBC (20) &     29\ 546 &     299\ 729 & \bf 802 & \bf 1\ 754 & \textit{OOM} &     0.552 &     0.967 \\
         & & \FISHDBC (50) & \bf 31\ 404 & \bf 299\ 757 &     888 &     1\ 924 & \textit{OOM} &     0.552 & \bf 0.968 \\
        %  & & 100 &     31\ 998 &     301\ 764 &     942 &     2\ 028 & &     0.547 & \bf 0.968 \\
        %  & & 200 & \bf 32\ 259 & \bf 301\ 792 &     963 &     2\ 076 & & \bf 0.543 & \bf 0.968 \\
        %  & &  NG &     29\ 758 &           -- &  4\ 818 &         -- & &     0.05  &     0.65  \\
         & &  \HDBSCAN & \oom \\
        \midrule
        % \multirow{2}{*}{DW-Pubmed} & \multirow{2}{*}{8\ 200\ 000} & 10 & 6\ 433\ 838 & 6\ 562\ 491 & 3 & 6\ 364 & & 0.979 & 0.989 \\
        %  & &  \HDBSCAN & \oom \\
        % \midrule
        \multirow{3}{*}{Finefoods} & \multirow{3}{*}{568\ 464}
        %   &  10 & \bf 159\ 572 &     567\ 892 &     3\ 031 &     7\ 008 & &     0.242 &     0.343 \\
           & \FISHDBC (20) &      77\ 152 &     566\ 484 & \bf 2\ 924 & \bf 6\ 262 & \textit{OOM} &     0.282 & \bf 0.372 \\
         & & \FISHDBC (50) &      79\ 904 &     568\ 104 &     3\ 531 &     7\ 486 & \textit{OOM} & \bf 0.226 &     0.363 \\
        %  & & 100 &      86\ 157 &     576\ 173 &     3\ 888 &     8\ 196 & &     0.233 &     0.362 \\
        %  & & 200 &      93\ 075 & \bf 568\ 236 &     4\ 156 &     8\ 760 & &     0.238 &     0.361 \\
        %  & &  NG &     324\ 425 &           -- &     9\ 691 &         -- & &     0.02  &     0.23 \\
         & &  \HDBSCAN & \oom \\
        \midrule
        \multirow{3}{*}{Household} & \multirow{3}{*}{2\ 049\ 280}
        %   &  10 &     1\ 459\ 303 &     2\ 048\ 639 &     14\ 828 &     62\ 548 & & \bf 1.59 &     13.84 \\
           & \FISHDBC (20) &     1\ 587\ 223 &     2\ 049\ 175 &     12\ 268 & \bf 61\ 582 & \textit{OOM} &     2.71 &     13.48 \\
         & & \FISHDBC (50) & \bf 1\ 649\ 304 &     2\ 049\ 224 & \bf 11\ 198 &     61\ 902 & \textit{OOM} &     2.76 &     13.17 \\
        %  & & 100 &     1\ 655\ 268 &     2\ 049\ 253 &     11\ 194 &     61\ 896 & &     2.84 &     13.34 \\
        %  & & 200 & \bf 1\ 675\ 048 &     2\ 049\ 254 & \bf 10\ 797 &     62\ 096 & &     2.88 &     13.43 \\
         & &  \HDBSCAN &     1\ 395\ 980 & \bf 2\ 049\ 273 &     53\ 358 &    173\ 198 & \textit{OOM} &    \bf 2.41 & \bf 13.94 \\
        %  & &  NG &     1\ 707\ 657 &              -- &     13\ 474 &          -- & &     0.5  &      0.53 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Internal clustering quality metrics. \textit{OOM} stands for out-of-memory errors when computing the Silhouette metric.}
    \label{tab:internal}
\end{table*}


==> figures/tab-runtime.tex <==
% tab:runtime
\begin{table}[thbp]
    \centering
    \begin{adjustbox}{max width=\columnwidth}
    \rowcolors{3}{gray!15}{white}
    \begin{tabular}{lrrrrr}
    \toprule
    \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{$\ef=20$} & \multicolumn{2}{c}{$\ef=50$} & \HDBSCAN \\
    & build & cluster & build & cluster & (accelerated?) \\
    \midrule
    % 20 Newsgroups & 106 & 0.471 & 303 & 0.435 & \textbf{13.0} (yes) \\
    % Blobs & \multicolumn{5}{c}{\textit{see \Vref{fig:blobs_runtime}}} \\
    % DW-Kos & 27.4 & 0.102 & 37.1 & 0.103 & \textbf{1.06} (yes) \\
    DW-Enron & 616 & 2.39 & 851 & 2.06 & \textbf{112} (yes) \\
    DW-NYTimes & \textbf{8\ 733} & 41.1 & 12\ 604 & 36.8 & \textit{OOM} (yes) \\
    % DW-Pubmed & \multicolumn{5}{c}{\textit{out of memory (results for $\ef=10$ in 12 days)}}\\
    Finefoods & \textbf{50\ 422} & 48.9 & 84\ 765 & 42.9 & \textit{OOM} (no) \\
    % Fuzzy hashes & \multicolumn{5}{c}{\textit{see \Vref{fig:fuzzy_runtime}}} \\
    Household & 27\ 375 & 123 & 38\ 759 & 109 & \textbf{24\ 258} (yes) \\
    % Synth & \multicolumn{5}{c}{\textit{see \Vref{tab:synth_runtime}}} \\
    USPS & 9.1 & 0.0500 & 12.1 & 0.0502 & \textbf{1.57} (no) \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Runtime (s). See \cref{tab:synth_runtime} for column description.}
    \label{tab:runtime}
\end{table}


